CXL Memory as Persistent Memory for Disaggregated HPC: A Practical Approach

In the landscape of High-Performance Computing (HPC), the quest for efficient and scalable memory solutions remains paramount. The advent of Compute Express Link (CXL) introduces a promising avenue with its potential to function as a Persistent Memory (PMem) solution in the context of disaggregated HPC systems. This paper presents a comprehensive exploration of CXL memory's viability as a candidate for PMem, supported by physical experiments conducted on cutting-edge multi-NUMA nodes equipped with CXL-attached memory prototypes. Our study not only benchmarks the performance of CXL memory but also illustrates the seamless transition from traditional PMem programming models to CXL, reinforcing its practicality. To substantiate our claims, we establish a tangible CXL prototype using an FPGA card embodying CXL 1.1/2.0 compliant endpoint designs (Intel FPGA CXL IP). Performance evaluations, executed through the STREAM and STREAM-PMem benchmarks, showcase CXL memory's ability to mirror PMem characteristics in App-Direct and Memory Mode while achieving impressive bandwidth metrics with Intel 4th generation Xeon (Sapphire Rapids) processors. The results elucidate the feasibility of CXL memory as a persistent memory solution, outperforming previously established benchmarks. In contrast to published DCPMM results, our CXL-DDR4 memory module offers comparable bandwidth to local DDR4 memory configurations, albeit with a moderate decrease in performance. The modified STREAM-PMem application underscores the ease of transitioning programming models from PMem to CXL, thus underscoring the practicality of adopting CXL memory.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> conf_table.tex <==
\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\diagbox[height=0.7cm,width=2cm]{\textbf{cores}}{\textbf{mem}} & \textbf{ Socket0} & \textbf{ Socket1} & \textbf{CXL} \\
\hline
\rule[-1ex]{0pt}{4ex}\textbf{Socket0}\rule[-1ex]{0pt}{4ex} & Local reference (one socket) & Remote reference (CXL Emulation) & Remote CXL \\
\hline
\rule[-1ex]{0pt}{4ex}\textbf{Socket1}\rule[-1ex]{0pt}{4ex} & Remote reference (CXL Emulation) & Local reference (one socket) & Remote CXL \\
\hline
\rule[-1ex]{0pt}{4ex}\textbf{Socket0+1}\rule[-1ex]{0pt}{4ex} & Local reference (all cores)& Local reference (all cores) & Remote CXL \\
\hline
\end{tabular}}
\vspace{0.5cm}
\caption{Confusion matrix of different hardware settings to experiment}
\end{table}

==> misc.tex <==
\begin{figure*}[t] % t: top of the page, b: bottom, h: here
    \centering
    
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cxl_copy.pdf}
        \caption{Copy STREAM for DDR5 and DDR4-CXL in system 1 (no HT, no FT)}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nvram001_copy.pdf}
        \caption{Copy STREAM for DDR4 in system 2 (no HT, no FT)}
        \label{fig:subfig2}
    \end{subfigure}
    
    \vspace{0.5cm} % adjust vertical spacing between rows
    
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cxl_scale.pdf}
        \caption{Scale STREAM for DDR5 and DDR4-CXL in system 1 (no HT, no FT)}
        \label{fig:subfig3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nvram001_scale.pdf}
        \caption{Scale STREAM for DDR4 in system 2 (no HT, no FT)}
        \label{fig:subfig4}
    \end{subfigure}
    
    \vspace{0.5cm} % adjust vertical spacing between rows
    
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cxl_add.pdf}
        \caption{Add STREAM for DDR5 and DDR4-CXL in system 1 (no HT, no FT)}
        \label{fig:subfig5}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nvram001_add.pdf}
        \caption{Add STREAM for DDR4 in system 2 (no HT, no FT)}
        \label{fig:subfig6}
    \end{subfigure}

        \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cxl_legend.PNG}
        \label{fig:subfig5}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nvram001_legend.PNG}
        \caption{...}
        \label{fig:subfig6}
    \end{subfigure}
    
    \caption{[NOTE:To remove in paper final version. Here for analysis]. STREAM with various hardware configurations}
    \label{fig:subfigures}
\end{figure*}


% We provide an in-depth overview of our CXL (Compute Express Link) prototype's implementation on an FPGA card. \autoref{fig:cxl_diagram}
% and \autoref{fig:system} grant a more detailed view into the implementation of our CXL memory pool on the FPGA card (while \autoref{fig:ddr4_node_diagram} show the reference system, without any cxl attachment, with DDR4 main memory). The prototype aims to harness the capabilities of the R-Tile Intel FPGA IP for CXL, encompassing critical functionalities for CXL link establishment and transaction layer management. This comprehensive solution facilitates the construction of FPGA-based CXL 1.1/2.0 compliant endpoint designs, including Type 1, Type 2, and Type 3 configurations.

% The architecture of our CXL implementation revolves around a synergistic pairing of protocol Soft IP within the FPGA main fabric die and the Hard IP counterpart, the R-Tile. This cohesive arrangement ensures effective management of CXL link functions, which are pivotal for seamless communication. Specifically, the R-Tile interfaces with a CPU host via a PCIe Gen5x16 connection, delivering a theoretical bandwidth of up to 64GB/s. As a key facet of our implementation, the FPGA device is duly enumerated as a CXL endpoint within the host system.

% Complementing this link management, the Soft IP assumes the mantle of transaction layer functions, vital for the successful execution of different CXL endpoint types. For Type 3 configurations, the CXL.mem transaction layer adeptly handles incoming CXL.mem requests originating from the CPU host. It orchestrates the generation of host-managed device memory (HDM) requests directed toward an HDM subsystem. Simultaneously, the CXL.io transaction layer undertakes the responsibility of processing CXL.io requests. These requests encompass both configuration space and memory space inquiries initiated from the CPU host, seamlessly forwarding them to their designated control and status registers. A noteworthy augmentation is the User Streaming Interface, offering a conduit for custom CXL.io features that can be seamlessly integrated into the user design.

% Integral to our FPGA card is the inclusion of two onboard DDR4 memory modules, each boasting a capacity of 8GB and operating at a clock frequency of 1333 MHz. These modules are accessible from the host system as conventional memory resources. It is imperative to highlight a distinctive attribute of this prototype configuration: the CXL link facilitates access to an identical memory volume. In essence, this means that the same far memory segment can be made available to two distinct NUMA nodes, eliminating any concerns of address overlap. However, due to the absence of a unified cache-coherent domain, the onus of maintaining coherency between the two NUMA nodes assigned to the shared far memory rests with the applications leveraging this configuration.

% Notably, the bandwidth attainable from this prototype configuration is subject to current implementation constraints and does not reflect an intrinsic limitation of the CXL standard. Potential avenues for enhancing bandwidth include several considerations. First, transitioning to a higher-speed FPGA, supporting DDR4 speeds of 3200 Mbps or even embracing the capabilities of DDR5 at 5600 Mbps, could appreciably enhance throughput. Additionally, scaling the resources allocated to the CXL IP by increasing the number of slices is a viable strategy. Furthermore, expanding the FPGA's capacity to accommodate multiple independent DDR channels, possibly transitioning from one channel to four, holds promise in augmenting the prototype's bandwidth potential.

% Lastly, it's noteworthy that the prototype's scalability is a key consideration. The aggregated bandwidth from interleaving multiple instances of these CXL-enabled FPGA devices stands as a testament to the extensibility of this solution, further reinforcing its utility in high-performance computing scenarios.

% In our discussion, it is worth noting that the fact that the CXL memory device is actually DDR4 and not DDR5 is key, as usually, PMem is slower and cheaper than the main memory. By using DDR4 CXL memory and not DDR5, while our main memory is DDR5, we keep on this important relation.


% We delve into the implementation of our CXL (Compute Express Link) prototype on an FPGA card, as showcased in Figures \ref{fig:cxl_diagram} and \ref{fig:system}. The prototype harnesses the R-Tile Intel FPGA IP for CXL, enabling essential CXL link establishment and transaction layer management. This inclusive solution facilitates FPGA-based CXL 1.1/2.0 compliant Type 1, Type 2, and Type 3 endpoint designs.

% The architecture combines protocol Soft IP within the FPGA main fabric die and the complementary R-Tile Hard IP. The R-Tile interfaces with a CPU host via PCIe Gen5x16, delivering up to 64GB/s bandwidth. The FPGA device assumes a CXL endpoint role within the host system.

% The Soft IP handles transaction layer functions. For Type 3 setups, the CXL.mem transaction layer manages incoming CXL.mem requests from the CPU host, generating host-managed device memory (HDM) requests to an HDM subsystem. The CXL.io transaction layer handles CXL.io requests, forwarding configuration and memory inquiries to designated control and status registers. The User Streaming Interface accommodates custom CXL.io features.

% The FPGA card integrates two 8GB DDR4 memory modules operating at 1333 MHz, accessible to the host. Notably, the CXL link provides access to the same memory volume, offering non-overlapping NUMA node access. Coherency between the NUMA nodes is application-dependent due to the lack of a unified cache-coherent domain.

% Prototype bandwidth is influenced by implementation constraints. Strategies for improvement include using faster FPGAs (DDR4 3200 Mbps or DDR5 5600 Mbps), scaling CXL IP resources, and expanding DDR channels (from one to four). The prototype's scalability is evident through bandwidth aggregation from interleaved CXL-enabled FPGA instances, exemplifying its applicability in high-performance computing. 

% In our discussion, it is worth noting that the fact that the CXL memory device is actually DDR4 and not DDR5 is key, as usually, PMem is slower and cheaper than the main memory. By using DDR4 CXL memory and not DDR5, while our main memory is DDR5, we keep on this important relation.


==> raw-materials.tex <==
\section{RAW MATERIALS TO PLACE IN CORRECT LOCATIONS}
\subsection{From NVRAM to CXL}

% Ref: https://www.intel.com/content/www/us/en/products/docs/memory-storage/optane-persistent-memory-to-cxl-attached-memory.html

Compute Express Link (CXL) emerges as a prospective alternative to Intel Optane Non-Volatile Random-Access Memory (NVRAM) due to its inherent potential to address the escalating demands for enhanced memory capacities, data transfer rates, and system performance within contemporary computing environments. As data-centric workloads continue to evolve, there is a pressing need to bridge the gap between traditional memory technologies and storage solutions. CXL, as an open standard interconnect, offers a memory-coherent and high-bandwidth connection between processors and memory devices, facilitating seamless integration of heterogeneous memory technologies. While Optane NVRAM has been pivotal in augmenting memory capacity beyond DRAM limitations, CXL introduces a comprehensive framework that encompasses not only memory expansion but also memory pooling, sharing, and hierarchical arrangements, thereby enabling a more holistic memory solution. The standardized nature of CXL assures compatibility across various hardware and software ecosystems, fostering interoperability and ease of adoption. This transition from Optane NVRAM to CXL is driven by the imperative to address the evolving needs of data-intensive workloads and unlock the potential for more sophisticated memory architectures, ultimately ushering in an era of heightened computational capabilities and system efficiency.


\subsection{CXL vs. NVRAM: A Comparative Analysis}

% Ref: https://arxiv.org/abs/2303.15375

\begin{table*}[h]
\centering
\caption{Comparison between CXL and NVRAM}
\begin{tabular}{|p{2.5cm}|p{7cm}|p{7cm}|}
\hline
\textbf{Aspect} & \textbf{CXL} & \textbf{NVRAM} \\
\hline
Bandwidth and Data Transfer & Significantly higher bandwidth enabling fast data transfers between processors and memory devices. & Non-volatile storage with potential data transfer rate limitations due to underlying interface and technology. \\
\hline
Memory Coherency & Provides memory-coherent links, ensuring consistent data across different memory tiers. & Requires additional mechanisms for memory coherency, except with local RAM, when integrated with other memory technologies. \\
\hline
Heterogeneous Memory Integration & Allows seamless integration of various memory technologies within a unified architecture. & Effective for extending memory capacity, but integration may require additional considerations due to unique characteristics. \\
\hline
Memory Pooling and Sharing & Facilitates memory pooling and sharing, enabling efficient resource utilization and dynamic allocation based on workload requirements. & Extends memory capacity, but inherent flexibility in memory sharing and pooling may be limited. \\
\hline
Industry Standardization & Open industry standard supported by major technology players, ensuring compatibility, interoperability, and broader adoption. & Solutions may vary, potentially leading to compatibility challenges and limited integration options. \\
\hline
Scalability & Architecture designed for scalability with multiple lanes and protocols, catering to evolving data center needs. & Scalability may be constrained by underlying technology characteristics, such as DIMM count and RAM/NVRAM tradeoff. \\
\hline
Relevance to HPC & Higher bandwidth, memory coherency, and memory pooling capabilities enhance HPC workload performance. Standardization ensures compatibility in heterogeneous environments, and scalability caters to evolving demands. & Offers non-volatility but constrained by limitations in bandwidth, coherency management, and scalability, affecting its applicability to complex HPC memory needs. Experimental evaluations highlight CXL's feasibility and performance as a superior persistent memory alternative in HPC systems. \\
\hline
\end{tabular}
\end{table*}


\subsection{PMDK with Optane and RAM}

% Ref: https://dl.acm.org/doi/abs/10.1145/3329785.3329930?casa_token=S5GwqxeORZ4AAAAA:_74rRMyIv2sLvtRNeObKdTxlfwnmIOnqQl1a8PP1P5_o_1aeGlutpHPcBzmpHQfC0-x66Upcp4B3M8Q

% Ref: https://dl.gi.de/items/ba3b1c7a-a5bc-4424-89fd-d4b8caa278a8

In the context of utilizing the Persistent Memory Development Kit (PMDK), the distinction between DRAM and PMem in App Direct mode lies in their access and performance characteristics. DRAM, as a traditional volatile memory, typically offers higher bandwidth and lower latency than PMem in App Direct mode. While PMem provides the advantage of persistence and larger capacity—e.g., PMem modules can reach capacities up to 512 GB per module—its access times and throughput are generally slower than DRAM. PMDK enables applications to harness PMem's persistence features, allowing data to be preserved across power cycles, while still accommodating the performance trade-offs associated with PMem's unique characteristics when compared to traditional DRAM. 
The experimental results revealed notable disparities in bandwidth between PMem and DRAM, with PMem exhibiting lower read bandwidth by a factor of 2.6 and write bandwidth by a factor of 7.5 compared to DRAM. Furthermore, in the context of write bandwidth, the introduction of additional threads actually led to a degradation in performance. Consequently, for performance-critical code, prioritizing DRAM over PMem is recommended as an optimization strategy—this could involve buffering writes within a DRAM cache to mitigate the impact of PMem's lower write bandwidth and potential thread-induced performance degradation.

\subsection{Battery-backed RAM and the appearance of Optane}

% Ref: https://www.cs.utexas.edu/~rak/papers/Dissertation.pdf

Battery-backed DRAM has been accessible from diverse vendors over a significant timeframe, representing an established concept. In a remarkable departure, Intel Optane DC persistent memory, which employs 3D XPoint technology, debuted in 2019. While diverse in characteristics, these NVMM technologies share a fundamental goal: delivering rapid byte-addressable data access alongside persistent data retention across power cycles. Often realized as non-volatile DIMMs (NVDIMMs), these technologies interface with the main memory bus in conjunction with DRAM. This integration optimizes access latencies, paralleling the speed of DRAM. 

\subsection{Disaggregated memory in HPC}

% Ref: https://arxiv.org/abs/2306.04014
% Ref: https://arxiv.org/abs/2305.05033
% Ref: https://dl.acm.org/doi/abs/10.1145/3529336.3530817
% Ref: https://ieeexplore.ieee.org/abstract/document/10024061?casa_token=6QFBysJPup8AAAAA:LVfLp-LRXufhkl0-Pi1eIdWwewhApcHfOVqG8GrTljNTDkS5gsGZ_PddaE6EmhxnBnUHsBujGpUK

The emergence of discrete memory nodes housing dynamic random-access memory (DRAM) and network interface controllers (NICs) is anticipated to revolutionize conventional memory paradigms, facilitating distributed memory access and reshaping HPC landscapes. This shift aligns with the concept of disaggregation, where compute resources and memory units are decoupled for optimized resource utilization, scalability, and adaptability. Leveraging advanced interconnect technologies such as Compute Express Link (CXL), memory nodes will be interconnected through high-speed links, enabling adaptive memory provisioning to compute nodes in real-time.  It is observed that the practice of intra-rack disaggregation holds the potential to effectively address the memory demands of applications while concurrently ensuring an adequate supply of remote memory bandwidth. % Ref: https://arxiv.org/abs/2301.03592
